Is Knowledge Power? On the (Im)possibility of Learning from Strategic Interactions

When learning in strategic environments, a key question is whether agents can overcome uncertainty about their preferences to achieve outcomes they could have achieved absent any uncertainty. Can they do this solely through interactions with each other? We focus this question on the ability of agents to attain the value of their Stackelberg optimal strategy and study the impact of information asymmetry. We study repeated interactions in fully strategic environments where players' actions are decided based on learning algorithms that take into account their observed histories and knowledge of the game. We study the pure Nash equilibria (PNE) of a meta-game where players choose these algorithms as their actions. We demonstrate that if one player has perfect knowledge about the game, then any initial informational gap persists. That is, while there is always a PNE in which the informed agent achieves her Stackelberg value, there is a game where no PNE of the meta-game allows the partially informed player to achieve her Stackelberg value. On the other hand, if both players start with some uncertainty about the game, the quality of information alone does not determine which agent can achieve her Stackelberg value. In this case, the concept of information asymmetry becomes nuanced and depends on the game's structure. Overall, our findings suggest that repeated strategic interactions alone cannot facilitate learning effectively enough to earn an uninformed player her Stackelberg value.

==> full-vs-partial.tex <==
\section{Perfect knowledge vs partial knowledge}
\begin{theorem}\label{AgentSignalLowerBound}
    For all $p_0\in[0,1)$, there exists a distribution $\cD$ over games such that $\forall p\le p_0$, all equilibrium $(\pi_1,\pi_2)$ in the algorithms space where $\pi_2$ has access to a signal of precision $p$ must satisfy $\Bar{U_2}(\pi_1,\pi_2)<\E_{G\sim \cD}[\stackval_2(G)]$.
\end{theorem}
\begin{proof}[Proof sketch]
\kycomment{will polish later}
    \begin{figure}[ht]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        $\begin{array}{c|cc}
        & C & D \\ 
        \hline
        A & \cellcolor{gray!50}16/\gamma, 1 & 16/\gamma, - 32/\gamma\\
        B & 2, 0 & 0, 2 \\
        \end{array}$
        \caption*{Game Matrix $G_1$}
    \end{minipage}
    \hspace{0.1\textwidth} %
    \begin{minipage}{0.4\textwidth}
        \centering
        $\begin{array}{c|cc}
        & C & D \\
        \hline
        A & 1, 1 & 0, -32/\gamma \\
        B & 4/5, 0 & 
        \cellcolor{gray!50}1/6, 2 \\
        \end{array}$
        \caption*{Game Matrix $G_2$}
    \end{minipage}
    \caption{game matrices $G_1$ and $G_2$. Shaded cells represent the action profiles supported in the Stackelberg equilibria led by the column player. The parameter $\gamma$ is defined as $\frac{1-p_0}{1+p_0}\in(0,1]$}
    \label[figure]{fig:full-vs-partial}
\end{figure}
Consider a given $p\le p_0$ and assume $(\pi_1,\pi_2)$ is an equilibirium that gives player 2 an average utility of at least $\E_{G\sim\cD}\stackval(G)$.
Let
\begin{align*}
    \T_1&\triangleq\frac{1+p}{2}\CSP(\pi_1(G_1),\pi_2(s_1))+\frac{1-p}{2}\CSP(\pi_1(G_1),\pi_2(s_2));\\
    \T_2&\triangleq\frac{1-p}{2}\CSP(\pi_1(G_2),\pi_2(s_1))+\frac{1+p}{2}\CSP(\pi_1(G_2),\pi_2(s_2)). 
\end{align*}
We have 
\begin{itemize}
    \item $\T_1((A,D))\le\gamma/8$, otherwise player 1 wants to deviate to $\pi_1'$ that always play action $A$.

    If $\T_1((A,D))>\gamma/8$, then 
    \begin{align*}
        \Bar{U}_1(\pi_1,\pi_2)&=
        \frac{1}{2}\Ex_{\tau\sim \T_1}\Bar{U}_1(\tau;G_1)
        +\frac{1}{2}\Ex_{\tau\sim \T_2}\Bar{U}_1(\tau;G_2)
        \\&<\frac{1}{2}\left(\frac{\gamma}{8}U_1((B,D);G_1)+\left(1-\frac{\gamma}{8}\right) U_1((A,C);G_1)\right)+\frac{1}{2}U_1((A,C);G_2)\\
        &=\frac{1}{2}\left(1-\frac{\gamma}{8}\right)\frac{16}{\gamma}+\frac{1}{2}\\
        &<\frac{1}{2}\cdot\frac{16}{\gamma}=\frac{1}{2}\Ex_{\tau\sim\T(\pi_1',\pi_2;G_1)}U_1(\tau;G_1)\\
        &\le \Bar{U}_1(\pi_1',\pi_2).
    \end{align*}
    \item $\T_1((A,C))\le\gamma/8$, otherwise player 2 wants to deviate to $\pi_2'$ that always plays action $C$.
    
    If $\T_1((A,C))>\gamma/8$, then
    \begin{align*}
        \Bar{U}_2(\pi_1,\pi_2)&=
        \frac{1}{2}\Ex_{\tau\sim \T_1}\Bar{U}_2(\tau;G_1)
        +\frac{1}{2}\Ex_{\tau\sim \T_2}\Bar{U}_2(\tau;G_2)\\
        &< \frac{1}{2}\cdot\frac{\gamma}{8}U_2(A,C)+
            \left(1-\frac{1}{2}\cdot\frac{\gamma}{8}\right)U_2((A,C))\\
        &=\frac{\gamma}{16}\cdot\left(-\frac{32}{\gamma}\right)+\left(1-\frac{\gamma}{16}\right)\cdot1\\
        &<0\le \Bar{U}_2(\pi_1,\pi_2').
    \end{align*}
    \item If $\T_2((B,D))\ge1/2$, otherwise player 2 cannot achieve the expected Stackelberg value benchmark.

    If $\T_2((B,D))<1/2$, then
    \begin{align*}
        \Bar{U}_2(\pi_1,\pi_2)&=
        \frac{1}{2}\Ex_{\tau\sim \T_1}\Bar{U}_2(\tau)
        +\frac{1}{2}\Ex_{\tau\sim \T_2}\Bar{U}_2(\tau)\\
        &\le  \frac{1}{2}\left(\left(1-\frac{\gamma}{8}\right)U_2(A,C)+\frac{\gamma}{8}\cdot U_2(B,D)\right)+\frac{1}{2}\left(\frac{1}{2}  U_2(A,C)+\frac{1}{2} \cdot U_2(B,D)\right)\\
        &<\frac{3}{2}=\E_{G\sim \cD}\stackval_2(G).
    \end{align*}
\end{itemize}
Finally, we show that if $\T_1,\T_2$ satisfies all the three bullet points above, then the principal gains utility by deviating to an algorithm $\pi_1'$ that always plays according to $G_1$, i.e., $\pi_1'(G_1)=\pi_1'(G_2)=\pi_1(G_2)$.
\begin{align*}
    \Bar{U}_2(\pi_1',\pi_2)-\Bar{U}_2(\pi_1,\pi_2)&=
        \frac{1-p}{4}\left(\Bar{U}_1(\sigma_1(G_1),\sigma_2(s_1);G_2)
        -\Bar{U}_1(\sigma_1(G_2),\sigma_2(s_1);G_2)
        \right)\\
        &\qquad
        +\frac{1+p}{4}\left(
        \Bar{U}_1(\sigma_1(G_1),\sigma_2(s_2);G_2)
        -\Bar{U}_1(\sigma_1(G_2),\sigma_2(s_2);G_2)\right)\\
        &=\frac{1}{2}\left(
        \frac{1-p}{2}\left(\Bar{U}_1(\sigma_1(G_1),\sigma_2(s_1);G_2)\right) 
        +\frac{1+p}{2}\left(\Bar{U}_1(\sigma_1(G_1),\sigma_2(s_2);G_2)\right) 
        \right)\\
        &\quad-
        \frac{1}{2}\left(
        \frac{1-p}{2}\left(\Bar{U}_1(\sigma_1(G_2),\sigma_2(s_1);G_2)\right) 
        +\frac{1+p}{2}\left(\Bar{U}_1(\sigma_1(G_2),\sigma_2(s_2);G_2)\right) 
        \right)\\
\end{align*}
For the first term, it is lower bounded by $\frac{1}{2}$ times
\begin{align*}
    &\quad\frac{1+p}{1-p}\cdot\T_1(\{(A,D),(B,D)\})
    \cdot U_1((A,D);G_2)
    +\left(1-\frac{1+p}{1-p}\cdot\T_1(\{(A,D),(B,D)\})\right)
    \cdot U_1((B,C);G_2)\\
    &\ge\left(1-\frac{1}{\gamma}\cdot\frac{\gamma}{4}\right)
    \cdot U_1((B,C);G_2)\tag{$\T_1(\{(A,D),(B,D)\})\le\frac{\gamma}{4}$ and $\frac{1+p}{1-p}\le\frac{1+p_0}{1-p_0}=\frac1\gamma$}\\
    &=\frac{3}{4}\cdot\frac{4}{5}=\frac{3}{5}
\end{align*}
For the second term, we can upper bound it by  $\frac{1}{2}$ times
\begin{align*}
   &\quad \T_2((B,D))\cdot U_1((B,D);G_2)+(1-\T_2((B,D)))\cdot U_1((A,C);G_2)\\
    &\le \frac{1}{2}\cdot U_1((B,D);G_2)+\frac{1}{2}\cdot U_1((A,C);G_2)
    \tag{$\T_2((B,D))\ge\frac{1}{2}$}\\
    \le&\frac{1}{2}\left(1+\frac{1}{6}\right)=\frac{7}{12}<\frac{3}{5}.
\end{align*}
Therefore, player 1's utility strictly increases after deviating from $\pi_1$ to $\pi_1'$. As a result, $(\pi_1,\pi_2)$ is not an equilibrium.
\end{proof}
